Equivariant Deep Dynamical Model for Motion Prediction

Learning representations through deep generative modeling is a powerful approach for dynamical modeling to discover the most simplified and compressed underlying description of the data, to then use it for other tasks such as prediction. Most learning tasks have intrinsic symmetries, i.e., the input transformations leave the output unchanged, or the output undergoes a similar transformation. The learning process is, however, usually uninformed of these symmetries. Therefore, the learned representations for individually transformed inputs may not be meaningfully related. In this paper, we propose an SO(3) equivariant deep dynamical model (EqDDM) for motion prediction that learns a structured representation of the input space in the sense that the embedding varies with symmetry transformations. EqDDM is equipped with equivariant networks to parameterize the state-space emission and transition models. We demonstrate the superior predictive performance of the proposed model on various motion data.

==> tex/exp.tex <==
\section{Experiment}
\section{Application}

\begin{itemize}
    \item 3D human action recognition (Recent
manifold-based approaches are quite successful at 3D human action recognition thanks to their view-invariant manifold-based representations for skeletal data.)
\end{itemize}


\subsection{Lie Group Representation for Skeletal Data}
From \textbf{\cite{huang2017deep}}:
Literature:
\begin{itemize}
    \item[\text{[3]}]R. Anirudh, P. Turaga, J. Su, and A. Srivastava. Elastic functional coding of Riemannian trajectories. IEEE T-PAMI, 2016.
    \item[\text{[41]}] R. Vemulapalli, F. Arrate, and R. Chellappa. Human action recognition by representing 3D skeletons as points in a Lie group. In CVPR, 2014.
    \item[\text{[42]}] R. Vemulapalli and R. Chellappa. Rolling rotations for recognizing human actions from 3D skeletal data. In CVPR, 2016.
\end{itemize}
\par 
Skeletal Data is collected through standard procedure as depicted in figure.~\ref{fig:skeletal}.
\begin{figure}[!h]
    \centering
    %\includegraphics[width=\linewidth]{figures/MoCap.jpg}
    \caption{Caption}
    \label{fig:skeletal}
\end{figure}

\par 
Let $S = (V,E)$ be a body skeleton, where $V =
\{v_1, \dots, v_N\}$ denotes the set of body joints, and $E = \{e_1, \dots, e_M\}$ indicates the set of edges, i.e. oriented rigid body bones (see figure.~\ref{fig:skelet}).

\begin{figure}[!h]
    \centering
    %\includegraphics[width=.6\linewidth]{figures/skelet.png}
    \caption{An example skeleton consisting of 20 joints and 19 body parts, (b) Representation of a body part $e_m$ in the global coordinate system.}
    \label{fig:skelet}
\end{figure}
Figure.~\ref{fig:skelet} shows an example
skeleton with 20 joints and 19 body parts. Let $e_{n1} \in \R^3$,
$e_{n2} \in \R^3$ respectively denote the starting and end points of
body part $e_n$. Let $l_n$ denote the length of $e_n$. Given a pair of body parts $e_m$ and $e_n$, to describe their relative geometry, we represent each of them in a local coordinate
system attached to the other. Figure.~\ref{fig:skCoor} explains this
pictorially. The local coordinate system of body part $e_n$ is obtained by rotating (with minimum rotation) and translating the global coordinate system such that $e_{n1}$ becomes the origin and $e_n$ coincides with the $x$-axis (refer to figure.~\ref{fig:skCoor}(a)).

\begin{figure}[!ht]
    \centering
    %\includegraphics[width0=.6\textwidth]{figures/sk_coordinate.png}
    \caption{Representation of body part $e_m$ in the local coordinate system of $e_n$, (b) Representation of body part en in the local coordinate system of $e_m$.}
    \label{fig:skCoor}
\end{figure}

Let $e_{m1}^n(t),e_{m2}^n\in\R^3$ respectively denote the starting and end points of $e_m$ represented in the local coordinate system attached to $e_n$ at time instance $t$. Then
\begin{equation}
    \begin{bmatrix}
    e_{m1}^n(t) & e_{m2}^n\\
    1 & 1 
    \end{bmatrix} = \begin{bmatrix}
    R_{m,n}(t) & \vec{d}_{m,n}(t)\\
    0 & 1 
    \end{bmatrix}\begin{bmatrix}
    0 & l_m\\
    0 & 0\\
    0 & 0\\
    1 & 1
    \end{bmatrix},
\end{equation}


where $R_{m,n}(t)$ and $\vec{d}_{m,n}(t)$ are the rotation and translation
(measured in the local coordinate system attached to $e_n$) required to take $e_n$ to the position and orientation of $e_m$.


\begin{itemize}
    \item Specifically, we can firstly calculate the axis-angle representation $(\boldsymbol{\omega}, \theta)$ for the rotation matrix $R_{m,n}$ by
\begin{align}
\bm{\omega} &= \frac{\hat{e}_m\otimes\hat{e}_n}{\norm{\hat{e}_m\otimes\hat{e}_n}}\\
        \theta &= \arccos(\hat{e}_m\cdot\hat{e}_n)
\end{align} 
    
    
    
    
    where $\otimes, \cdot$ are outer and inner products respectively. Then, the axis-angle representation can be easily transformed to a rotation matrix $R_{m,n}$.
    \item As a result, a skeleton $S$ at the time instance $t$ is represented by the form $(R_{1,2}(t),R_{2,1}(t) \dots ,R_{M-1,M}(t),R_{M,M-1}(t))$, where $M$ is the number of body parts, and the number of rotation matrices is $2\binom{M}{2}$.
\end{itemize}

%\norm{ \biggl(\sum_{n=1}^N \mathbf{P}_{n}\biggr) }








==> tex/extra.tex <==
%\textcolor{blue}{Most importantly, our experiments show that incorporating the  these two  of these together(initializations;  +  penalty;  method forthe latter) works well on real data yielding significant performance dividends interms of both speed and accuracy (c.f. Section 5). This too we believe isnon-obvious, and important to report to the broader community.}
